Towards Runtime Verification of Programmable Switches

Is it possible to patch software bugs in P4 programs without human involvement? We show that this is partially possible in many cases due to advances in software testing and the structure of P4 programs. Our insight is that runtime verification can detect bugs, even those that are not detected at compile-time, with machine learning-guided fuzzing. This enables a more automated and real-time localization of bugs in P4 programs using software testing techniques like Tarantula. Once the bug in a P4 program is localized, the faulty code can be patched due to the programmable nature of P4. In addition, platform-dependent bugs can be detected. From P4_14 to P4_16 (latest version), our observation is that as the programmable blocks increase, the patchability of P4 programs increases accordingly. To this end, we design, develop, and evaluate P6 that (a) detects, (b) localizes, and (c) patches bugs in P4 programs with minimal human interaction. P6 tests P4 switch non-intrusively, i.e., requires no modification to the P4 program for detecting and localizing bugs. We used a P6 prototype to detect and patch seven existing bugs in eight publicly available P4 application programs deployed on two different switch platforms: behavioral model (bmv2) and Tofino. Our evaluation shows that P6 significantly outperforms bug detection baselines while generating fewer packets and patches bugs in P4 programs such as switch.p4 without triggering any regressions.

==> sections/OLD-sections/OLD-challenges.tex <==

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/P4_bug_examples-crop.pdf}
    \caption{Example of a target device-independent (yellow) and -dependent (green) bug in \new packet processing pipeline.}
    \label{fig:mot2}
\end{figure*}


\section{Challenges \& Opportunities}\label{sec:challenges}
\subsection{Challenges: Bugs}

\begin{comment}
\begin{figure}[t]
\centering
%\includegraphics[width=\linewidth]{figures/scenario_v5-crop.pdf}
\includegraphics[width=\columnwidth]{figures/figure_ex_new7-crop.pdf}
\caption{Example of a target device-independent bug.}
%\ap{Make queries in different colour}}
\label{fig:mot}
%\ap{Font looks too small so make sure it is readable by naked eye. Use clker.com for free images which are not copyright}
\end{figure}
\end{comment}
In this section, we motivate the need for a runtime P4-switch verification system. 
%We, revisit two example scenarios from~\cite{shukla2} in the two publicly available P4 programs: \texttt{basic.p4}~\cite{p4tut}, and \texttt{acceptor.p4}~\cite{netp} running on a P4 switch. 
We illustrate the anomalies in the switch behavior due to missing checks in the publicly available P4 programs from P4 tutorial solutions~\cite{p4tut} and NetPaxos~\cite{netp} codebase.
 
%In this section we show a small example of some simple possible errors in a P4 program can have a critical effects even on the security of the system. Such a  problem may appear in syntactically correct, perfectly running code. If the P4 target device acts as a firewall, we can safely assume that it uses some kind of acl to filter traffic. As P4 programs execute actions on a packet based on a match-action tables. In Figure \ref{fig:missplacedacl} we can see a miss-placed application of the acl. In this case the acl will only apply to packets with valid IPv$4$ headers. This way IPv$6$ packets could be used to start an attack against the defended network.
%However, this is not the only problem regarding the code snippet in Figure \ref{fig:missplacedacl}. As "if" statements cannot be used in actions in P$4$, some additional considerations should take place on the mentioned figure. If an attacker intercepts and modifies an encrypted packet meant for the system in question, the checksum value most probably will be wrong. However, as the firewall do not check this value (there is no "if" statement regarding this particular field), the firewall will forward it and correct the checksum, legalizing the packet. This gives an opportunity to an attacker to insert malicious pieces of code or information, and get it to the system without any problems. 
%To the best of our knowledge, such scenarios are non-trivial to debug by any of the existing static analysis-based P4 program debugging approaches~\cite{stoenescu2018debugging,liu2018p4v,neves2018verification}.Scenarios like checksum-related bugs (see Example Scenario 1) are non-trivial to debug by any of the existing static analysis-based P4 program debugging approaches~\cite{stoenescu2018debugging,liu2018p4v,neves2018verification}. TTL-related bugs (see Example Scenario 2) can be, however, detected by~\cite{stoenescu2018debugging,neves2018verification}Such scenarios can be easily reproduced in the official P4 tutorial program~\cite{p4tut}, e.g., \texttt{basic.p4} and the NetPaxos P4 program~\cite{netp}, e.g., \texttt{acceptor.p4}.

Software bugs or errors can occur at any stage in the P4 processing pipeline: parser, ingress match-action, packet replication engine (\texttt{PRE}), egress match-action, deparser and buffer queuing engine ((\texttt{BQE}). Note all stages except the PRE and BQE, are P4 programmable while PRE and BQE remain as a vendor specific, fixed function component. Figure~\ref{fig:mot2} illustrates the target device-dependent (in green) and -independent (in yellow) blocks in the \new packet processing pipeline. Note that the target device-independent blocks are programmable.

There can be, however, bugs in the parser code, e.g., when not or incorrectly checking the header fields, such as IPv4 header length (\texttt{ihl}) or \texttt{TTL} field. 
%In case the programmer, e.g., forgets to verify TTL field is greater than 0, decrementing the TTL results in a TTL of 255. 
%The checksum validation block in ingress match-action also possesses weaknesses, possibly accepting packets with wrong checksums.
% In case the programmer, e.g., does not choose to parse IPv4 packets with options, the resulting checksum calculation will be wrong, leading to packet drop at other hops in the network. 
As an example, consider the scenario in Figure~\ref{fig:mot2} (yellow blocks) that illustrates part of the implementation of L3 (Layer-3) switch, provided in the P4 language tutorial solutions~\cite{p4tut}. Here, the parser accepts any kind of IPv4 packets and does not check if the IPv4 header contains IPv4 options or not, i.e., if IPv4 \texttt{ihl} field is not or is equal to 5. When updating the IPv4 \texttt{checksum} of the packets during egress processing, IPv4 options are not taken into account, hence for those IPv4 packets with options, the resulting \texttt{checksum} is wrong causing such packets to be \textit{incorrectly} forwarded instead of getting dropped. This leads to anomaly in the network behavior.
%Therefore, the next hop in the network expected to drop such packets does not drop them, leading to anomaly in the network behavior. 
Currently, the detection of such runtime bugs is non-trivial. We call such errors as \textit{target device-independent bugs}, as these only result from programming errors involving one of the P4 programmable stages. 

These are, however, not the only kind of bugs that can occur. The interaction of the P4 program with the \texttt{PRE} may result in an unintended behavior as well, which we call as \textit{target device-dependent bugs}. The \texttt{PRE} is responsible for carrying out several forwarding actions, such as \texttt{clone}, \texttt{multicast}, \texttt{resubmit} or \texttt{drop}. The programmer uses standard metadata to communicate the forwarding action to the \texttt{PRE}, which interprets it and executes the actions accordingly. It is, however, very common to have situations where conflicting forwarding actions are selected. %Consider a scenario where a P4 program implementing at least two tables, where one could be an IPv4 longest prefix match (\texttt{LPM}) table and a following table an access control list (\texttt{ACL}). If packets are matched by the \texttt{LPM} table and a clone decision is made, those packets later, get dropped by the \texttt{ACL} table. In such a case, the forwarding behavior depends on the implementation of the \texttt{PRE}, which is target device-dependent. The implementation of \texttt{PRE} of the simple switch target in the behavioral model (Bmv2) would drop the original packet, however, \textit{incorrectly} forward the cloned copy of the packet. Similar runtime bugs can be seen, if instead of \texttt{clone}, \texttt{multicast} or \texttt{resubmit} actions are chosen.
As an example, consider the scenario shown in Figure~\ref{fig:mot2} (green blocks). Here, we assume a P4 program implementing at least two match-action tables. Any table except the last one could be a longest prefix match (\texttt{LPM}) table, offering unicast, clone and drop actions. The last match-action table implements an access control list (\texttt{ACL}). So, the packets can either be dropped or forwarded according to the chosen actions by the previous tables. In this case, it is possible that conflicting forwarding decisions are made. Consider packets matched by the first table and a clone decision is made, are later dropped by the \texttt{ACL} table. In such a case, the forwarding behavior depends on the implementation of the \texttt{PRE}, which is target device-dependent. The implementation of \texttt{PRE} of the simple switch target in the behavioral model (Bmv2) is illustrated in Figure~\ref{fig:mot2}. It would drop the original packet, however, forward the cloned copy of the packet. Similar bugs can be seen, if instead of the clone action, the resubmit action is chosen (in blue). Similarly, another bug can be found when implementing multicast (in green). 
%Furthermore, if the programmer does not decide to choose a forwarding action at all, the value of the \texttt{egress\_spec} field is undefined as per $P4_{16}$ specification~\cite{p4-specs}. Therefore, the hardware implementing \texttt{PRE} is allowed to return an arbitrary value for the \texttt{egress\_spec}, thus defining an arbitrary output port for such packets. 

\ap{Check}Target device-independent or -dependent bugs are present in many real-world P4 applications. Currently, some of the aforementioned runtime bugs such as checksum-related bugs and platform-dependent bugs cannot be detected by the existing static analysis approaches~\cite{stoenescu2018debugging,liu2018p4v,neves2018verification,Neves:2018:VPP:3281411.3281421}.

\begin{figure*}[t]
\centering
\begin{subfigure}[l]{0.5\columnwidth}
\centering
\includegraphics[width=\columnwidth, height=4cm]{figures/p4_newest.pdf}
%\vspace{-.25em}
\subcaption{The patchable percentage of code increases for each P4 program from \old to \new. This plot is for bmv2 switch architecture~\cite{bmv2}, i.e., it does not include explicit ingress deparser and egress parser. \label{fig:apps}}
%\vspace{-.25em}
\end{subfigure}%
\hspace{0.01\textwidth}
\begin{subfigure}[c]{0.5\columnwidth}
\centering
\includegraphics[width=\columnwidth, height=4cm]{figures/p4_explicit_new.pdf}
%\vspace{-.25em}
\subcaption{The patchable percentage of code increases for each P4 program from \old to \new. This plot is for generic PSA switch architectures~\cite{psasec,psaing} like Tofino~\cite{tofino}, i.e., includes explicit ingress deparser and egress parser.\label{fig:apps1}}
%\vspace{-.25em}
\end{subfigure}%
\hspace{0.01\textwidth}
\begin{subfigure}[r]{0.5\columnwidth}
\centering
\includegraphics[width=\columnwidth, height=4cm]{figures/bargraph_newest.pdf}
%\vspace{-.25em}
\subcaption{The patchable percentage of code for bmv2 switch architecture~\cite{bmv2}, i.e., it does not include explicit ingress deparser and egress parser in all different \new programs from P4 tutorials~\cite{p4tut}, NetPaxos~\cite{netp}.\label{fig:per}}
%\vspace{-.25em}
\end{subfigure}
\hspace{0.01\textwidth}
\begin{subfigure}[r]{0.5\columnwidth}
\centering
\includegraphics[width=\columnwidth, height=4cm]{figures/bargraph_explicit_new.pdf}
%\vspace{-.25em}
\subcaption{The patchable percentage of code for generic PSA switch architectures~\cite{psasec,psaing} like Tofino~\cite{tofino}, i.e., includes explicit ingress deparser and egress parser in all different \new programs from P4 tutorials~\cite{p4tut}, NetPaxos~\cite{netp}. \label{fig:per1}}
%\vspace{-.25em}
\end{subfigure}
\caption{Evolution of the P4 program structure from \old to \new version. Note calculator (calc) application from~\cite{p4tut} is not included here as it not a networking application.}
\label{fig:struct}
\vspace{.5em}
\end{figure*}
\begin{comment}
\begin{figure}[t]
\centering
%\includegraphics[width=\linewidth]{figures/scenario_v5-crop.pdf}
\includegraphics[width=0.9\columnwidth]{figures/figure_clone_v8-crop.pdf}
\caption{Example of a target device-dependent bug.}
%\ap{Make queries in different colour}}
\label{fig:mot2}
\end{figure}
\end{comment}
\subsection{Opportunities: Structure of a P4 program}
P4~\cite{bosshart2014p4,p416specs} is a domain-specific language comprising of packet-processing abstractions, e.g., headers, parsers, tables, actions, and controls. A simple abstract forwarding model is followed with five distinct
phases while executing a P4 program: \texttt{parsing}, \texttt{ingress processing}, \texttt{replication} and \texttt{queuing},
\texttt{egress processing}, and \texttt{deparsing}~\cite{bosshart2013forwarding}. The behavior of each of these phases is defined through declarations in a P4 program. 

The parser transforms the packet from bits into headers according to a parser specification provided by the programmer. After parsing, an ingress control function decides how the packet will be processed. Then, the packed is queued for egress processing. Upon dequeuing, it is processed by an egress control function. The deparser specification dictates how packets are deparsed from separate headers into a bit representation on output, and finally, the packet leaves the switch. Note that both ingress and egress control functions direct the packet through any number of match-action tables. Figure~\ref{fig:mot2} illustrates these stages of the P4 packet processing pipeline.%The control functions conditionally steer the packet to various tables based on header values, metadata or table match outcomes. %; packet contents cannot be changed in the control function. %During execution, the state comprises the data extracted from packet headers, metadata supplied by the device (e.g., the ingress port that the packet arrived on) or computed by the program, as well as mutable state in counters and registers.

Currently, P4 offers 2 versions: \old~\cite{p414specs} and \new~\cite{p416specs}. \new allows programmers to use definitions of a target switch-specific architecture, PSA (Portable Switch Architecture)~\cite{psasec,psaing} which is a target architecture that describes common capabilities of network switch devices. \new is an upgraded version of \old. In particular, a large number of language features have been eliminated from \old and moved into libraries including counters, checksum units, meters, etc. in \new. \old allowed the programmer to explicitly program three blocks: ingress parser (including header definitions of accepted header layouts), ingress control and egress control functions. As illustrated in Figure~\ref{fig:mot2}, \new allows to explicitly program six blocks: ingress parser (including header definitions of accepted header layouts), ingress control, ingress deparser, egress parser, egress control functions, and egress deparser.

We realize that as more blocks of the P4 program get programmable, there is more onus on the programmer to write a program that behaves as expected when it gets compiled and is deployed on the P4 switch. However, missing checks or manual errors can cause havoc in the network. However, this is also a blessing in disguise as the more programmable the code is, the more patchable it gets. Thus, the manual errors can be fixed. Figure~\ref{fig:per},~\ref{fig:per1} illustrate that the patchable code percentage increases from \old to \new in all applications (excluding calculator) from P4 tutorial solutions~\cite{p4tut} and NetPaxos codebase~\cite{netp} in behavioral model (bmv2) switch architecture~\cite{bmv2} and other generic PSA switch architectures~\cite{psasec,psaing}, e.g., Tofino~\cite{tofino} respectively.\\ 
\emph{\textbf{Observation 1:} From} \old \emph{to} \new, P4 \emph{program gets more complex as there are twice as more programmable blocks.}

Figure~\ref{fig:apps},~\ref{fig:apps1} illustrate the patchable code percentage in the latest \new version. The patchable code percentage comes from the six programmable blocks in \new. Roughly, whatever is programmable, is patchable. In particular, around 40-45\% of a P4 program is patchable in \new programs for behavioral model (bmv2) switch architecture~\cite{bmv2} (Figure~\ref{fig:apps}). This increases to 50-55\% if the ingress deparser and egress parser is programmable for other target switch architectures, e.g., Tofino~\cite{tofino} (Figure~\ref{fig:apps1}). More importantly, the parser and header definitions account for 20-40\% of the total patchable code. Therefore, if there is no bug in the parser and header code, the runtime behavior of the switch running the compiled P4 program to the incoming packets should more or less behave as expected.\\ 
\emph{\textbf{Observation 2:} Parser code is patachable if localized; else the unexpected incoming traffic may get rejected anyway; otherwise the bug lies in the target-device dependent part or other parts of P4 code.} 

%see Figure~\ref{fig:per}\\
\begin{comment}
\begin{figure}[t]
\centering
%\includegraphics[width=\linewidth]{figures/apps.jpg}
\includegraphics[width=\columnwidth]{figures/p4_new.pdf}
\caption{The patchable percentage of code increases for each P4 program from \old to \new.}
%\ap{Make queries in different colour}}
\label{fig:apps}
\end{figure}
\begin{itemize}
    \item \new allows to explicitly program parser and deparser of the different stages (Ingress/ Egress) in the processing pipeline.
    \item Depending on the switch architecture the programmer needs to explicitly program both parser and deparser for each stage, ingress and egress.
    \item E.g. portable switch architecture (PSA) requires to explicitly program ingress parser, ingress deparser, egress parser and egress deparser~\cite{psaing,psasec}
    \item Bmv2 simple switch architecture is based on an architecture model that only requires the programmer to program ingress parser and egress deparser.
\end{itemize}
%see Figure~\ref{fig:apps}\\

%\emph{\textbf{Observation3:} other parts of code}

\begin{figure}[t]
\centering
%\includegraphics[width=\linewidth]{figures/Percent.jpg}
\includegraphics[width=\columnwidth]{figures/bargraph_new.pdf}
\caption{The patchable percentage of code in ten different \new programs from P4 tutorials~\cite{p4tut} and NetPaxos~\cite{netp} codebase.}
%\ap{Make queries in different colour}}
\label{fig:per}
\end{figure}
\end{comment}


==> sections/OLD-sections/OLD-introduction.tex <==
\section{Introduction}
\gs{What is programmable networks; p4 is software}
Recently, in the field of networking, there is a surge of softwarization or programmability. The network devices on the data plane, e.g., switches have become programmable which were traditionally, having fixed functionality or were dependent on a vendor-specific fixed-function proprietary hardware and software. Programmability of network devices, e.g., switches with the introduction of P4 language~\cite{bosshart2014p4, p416specs} has enabled the customization of the fixed data plane functionality. While the programmability enables to break the tie between vendor-specific hardware and proprietary software, it facilitates an independent evolution of the software and hardware. With the P4 language, one can define in a P4 program or source code, the instructions for processing the packets, e.g., how the received packet should be read, manipulated, and forwarded by a network device, e.g., a switch. Nevertheless, with the new capabilities, new challenges in switch verification have been unleashed.

\gs{Pose the question: three parts; detection, localization, patching}
%\smartparagraph{Many problems can happen at runtime in P4:} 
We pose the following question: \emph{``Is it possible to automatically \texttt{detect}, \texttt{localize}, and \texttt{patch} the software bugs in a P4 program without any human involvement?''} Since, the P4 switch behavior is dependent on the \emph{correctness} of the P4 programs running on those switches, we realize that a small bug, or an error, e.g., a missing line of code can trigger unexpected and abnormal switch behavior, or in the worst case, result in a network outage or even a security compromise. Lately, a plethora of verification systems~\cite{stoenescu2018debugging,liu2018p4v,neves2018verification,Neves:2018:VPP:3281411.3281421,Notzli:2018:PAT:3185467.3185497,shukla1,shukla2,shukla3} has been proposed for verification in P4 programs. Those verification systems, however, fail to automatically repair the P4 program containing bugs.

\gs{detection: static analysis; find bugs in compiler time with high cost} 
%\smartparagraph{Network behavior is runtime behavior of a P4 program and existing tools do static analysis and fail:} 
 Recently, a panoply of P4 program verification tools~\cite{stoenescu2018debugging,liu2018p4v,neves2018verification,Neves:2018:VPP:3281411.3281421} has been developed. These tools, however, mostly aim to statically verify user-defined P4 programs which are compiled to run on a target switch. Thus, they are prone to false positives and are unable to verify the runtime behavior on real packets. In addition, bugs like checksum-related bugs or platform-dependent bugs cannot be detetcted by static analysis approaches. \gs{runtime helps to detect bugs only when the pre-compiled code is deployed}
%\smartparagraph{Fuzzing is a solution but challenging, detection and localization are challenging:} 
While the runtime verification aims to verify the behavior of a switch by passing specially-crafted input packets to the switch and observing the behavior, the detection of bugs causing the abnormal runtime behavior can be a complex and challenging task as the P4 switch does not throw runtime exceptions. To give an example, if an uninitialized header value is read, the packets are either dropped silently or a random value is returned. Similarly, reading or writing an invalid header can produce arbitrary results~\cite{p416specs}. The behavior of a P4 switch, however, is not just determined by the P4 program but also the match-action table rules that are installed either by the controller at runtime, or statically, when the P4 program is deployed. In addition, the detection of bugs can be a nightmare if there is no output, i.e., packets are silently dropped instead of being forwarded. Thus, the runtime verification of the switch behavior is crucial. Recently,~\cite{shukla1, shukla2, shukla3} tried to tackle the P4 runtime verification, however, all fail to patch the bugs in the P4 source code.%Existing verification tools~\cite{stoenescu2018debugging,liu2018p4v,neves2018verification} perform static analysis on the P4 source program 

\gs{Very recently authors showed that fuzzing is a powerful tool}
A useful approach to verify the runtime behavior is fuzz testing or fuzzing~\cite{afl, lib, shukla2019consistent, shukla2, shukla3}, a well-known dynamic program analysis technique that generates semi-valid, random inputs which may trigger abnormal program behavior. However, for fuzzing to be efficient, intelligence needs to be added to the input generation, so that the inputs are not rejected by the parser and it maximizes the chances of triggering bugs. This becomes crucial especially in networking, where the input space is huge and complex, e.g., a 32-bit destination IPv4 address field in a packet header has $2^{32}$ possibilities. With the 5-tuple flows, the input space is even more complex.
In order to make fuzzing more effective, we consider the use of machine learning, to guide 
the fuzzer to generate smart inputs which trigger abnormal program behavior. 

\ap{machine-learning and static analysis}In recent years, artificial intelligence and machine learning have gained attention to solve very complex problems, also in the area of networking \cite{dumb, deepconf, shobha}. A variety of algorithms and approaches exist, which can be mainly categorized into supervised, semi-supervised, unsupervised and reinforcement learning \cite{Russell:2009:AIM:1671238}. %The goal of the supervised learning is to learn a function, which maps input to output, or labelling data into known classes, given examples of these mappings. Unsupervised learning on the other hand, aims at finding patterns in data without having examples and known labels. Semi-supervised learning is a combination of supervised and unsupervised learning methods. 
In contrast to the other approaches, reinforcement learning aims at enabling an agent to learn how to interact with an environment, based on a series of reinforcements, meaning rewards or punishments received from the target environment. The agent observes the environment and chooses an action to be executed. After the action is executed, the agent receives a reward or punishment from the environment. %The goal of learning is to maximize the received rewards and generalize from the learning experiences.
While the goal of learning is to maximize the rewards, we argue it is equally crucial to design a machine learning model which is general enough for any kind of target environment. To detect the bugs triggered by fuzzing, one can observe the output of the target device in response to the input packets. Recently, \cite{shukla2} showed machine-learning guided fuzzing and \cite{shukla3} showed static analysis-guided fuzzing, we improve \cite{shukla2} by augmenting the fuzzing with static analysis of the P4 program to make the fuzzing more focused and effective. The static analysis of the P4 program makes the fuzzer aware of the supported header layouts, e.g., IPv4, IPv6, etc. and thus, significantly reduce the input search space.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/P4_bug_examples-crop.pdf}
    \caption{Example of a target device-independent (yellow) and -dependent (green) bug in \new packet processing pipeline.}
    \label{fig:mot2}
\end{figure*}
\gs{localization}
 Furthermore, the localization of bugs in a P4 program can be cumbersome and time-consuming as the practical P4 programs can be large with a dense conditional structure. In addition, the same faulty statement/s in a P4 program may be executed for both: passed as well as failed test cases. Recently,~\cite{shukla2} tried to tackle the localization of bugs in a P4 program by using Tarantula-based fault localization~\cite{jones2001visualization, jones2002visualization, jones2005empirical}, however, it fails to take corrective actions like automatic patching of the bugs in the P4 program.

We realize, however, the automatic code repair (source code patching) is an uncharted territory. In this paper, we show that due to the structure of P4 programs, it is possible to automatically patch the P4 program or source code without human involvement. %In the process of triggering the patching process, and be backward-compatible, we significantly improved both detection and localization of bugs. In particular, the fuzzing of \cite{shukla2, shukla3} was improved to make bug detection and thus, localization and patching faster.% 
To this end, we present \system, \textbf{\emph{P4}} with automatic runtime \textbf{\emph{P}}rogram \textbf{\emph{P}}atching, a novel runtime P4-switch verification system that \emph{automatically} \texttt{detects}, \texttt{localizes}, and \texttt{patches} software bugs in a P4 program. \system improves the existing work based on machine learning-guided fuzzing~\cite{shukla2} and static analysis-guided fuzzing with localization~\cite{shukla3} in P4 by extending it and augmenting automatic runtime patching to it. \system relies on the combination of static analysis of the P4 program and reinforcement learning technique to guide the fuzzing process to verify P4 switches at runtime. 
%Using well-known machine learning techniques \cite{Hasselt:2016:DRL:3016100.3016191} can guide fuzzing in order to know what kind of program input is valuable or smart, and use that knowledge to control the input generation process. 
Using Double Deep Q Networks (DDQN)~\cite{Hasselt:2016:DRL:3016100.3016191}, we ensure that the evaluation of an action is independent of the selection of an action. Thus, we avoid the problem of overfitting for a given target environment. Furthermore, the prioritized experience replay~\cite{schaul2015prioritized} helps to avoid oscillations or divergence of parameters in the machine learning \agent. In addition, to specify the intended network behavior, e.g. P4 switch, we provide an easy-to-use query language, \lang, so that users can conveniently specify the \textit{expected} packet processing behavior in the conditional if-else statements and verify such behavior against the \textit{actual} behavior. \lang works in conjugation with \system. %Given the P4 source code and user-specified inputs, \system automatically generates test packets through fuzzing to trigger abnormal or unexpected behavior in the P4 switch. 
If an abnormal behavior is triggered, the feedback is used to guide the fuzzing process even further. When an anomaly or bug is detected by \system , the bug localization mechanism: \tar, based on Tarantula fault localization technique~\cite{jones2001visualization,jones2005empirical,jones2002visualization}, is \emph{automatically} activated to localize the potential problematic source code area. The localization process automatically triggers the patching process to patch the software bugs in the P4 program and then, compiles and deploys the P4 program on the P4 switch. The program is then tested to confirm the fixes or patches in addition, it does regression testing to ensure no regression was caused by the fixes. We designed \system with four main properties in mind: (a) \emph{expressivity} via user-specified options, e.g., IPv4 checksum, TTL, etc. to be tested; (b) detection; (c) localization of bugs in P4 programs; and (d) patching of bugs. To summarize, \system combines user input-, static analysis-, and reinforcement learning-guided fuzzing through \fuzz to speed up the bug detection and later, the dynamic program analysis by \tar for the localization of the detected bugs to be finally, patched by the \pat.

%\smartparagraph{\system prototype and results:}
We develop a prototype of \system and evaluate it by testing it on ten \new application programs from P4 tutorial solutions~\cite{p4tut}, and the NetPaxos codebase~\cite{netp} on two P4 architectures: Behavioral Model version 2 (bmv2)~\cite{bmv2} and Tofino~\cite{tofino}. Our results show that \system successfully detects, localizes and patches diverse bugs in all \new programs while significantly outperforming baseline approaches and not introducing any regressions by patching.\\ %Our results show that \system can detect and localize a panoply of software bugs or errors in a P4 program.% or in the control plane configuration. 
%revisit before submission
%Furthermore, our detailed performance and accuracy analyses show that %the verification time grows exponentially with the number of tables, \system needs less than x minutes to verify the two P4 applications.
%The three main challenges in the design of \system are: 1)fuzzing: huge space to attack 2) p4 bug detection: it is hard to detect bugs as the packets causing the bugs gets dropped silently 3) localization: most of the packets execute the same lines of code, but we have to find the faulty ones.
\textbf{\textit{Main Contributions.}} Our main contributions are:\\
%\begin{tcolorbox}
$\bullet$ We propose the first fully automated runtime verification P4 system, called \system. \system detects, localizes, and patches P4 programs without human involvement.\\
$\bullet$ Our solution relies on the observation that the patchable section of the P4 programs is well structured, thus, easy to automatically repair. We confirm this by studying XX code in two different P4 versions.\\
$\bullet$ We develop and evaluate our \system prototype on a P4 switch running ten \new programs from~\cite{p4tut,netp} in two P4 architectures, namely, Tofino~\cite{tofino} and Behavioral Model~\cite{bmv2}. We show that it is possible to automatically patch the detected bugs.\\
$\bullet$ Our results show that \system can automatically detect, localize and patch diverse bugs at runtime. In addition, \system outperforms the baseline bug detection approaches by upto x times.\\
$\bullet$ \system reduces the bug detection and localization time when compared to baseline approaches. We show that machine learning guided fuzzing can significantly boost the detection time with minimal packet generation overhead. \\
%%%%%%%
$\bullet$ \system software and a library of readymade patches for all bugs and P4 programs discussed in this paper will be made publicly available.
%\end{tcolorbox}

\section{Challenges \& Opportunities}
\subsection{Challenges: Bugs}

\begin{comment}
\begin{figure}[t]
\centering
%\includegraphics[width=\linewidth]{figures/scenario_v5-crop.pdf}
\includegraphics[width=\columnwidth]{figures/figure_ex_new7-crop.pdf}
\caption{Example of a target device-independent bug.}
%\ap{Make queries in different colour}}
\label{fig:mot}
%\ap{Font looks too small so make sure it is readable by naked eye. Use clker.com for free images which are not copyright}
\end{figure}
\end{comment}
In this section, we motivate the need for a runtime P4-switch verification system. %We, revisit two example scenarios from~\cite{shukla2} in the two publicly available P4 programs: \texttt{basic.p4}~\cite{p4tut}, and \texttt{acceptor.p4}~\cite{netp} running on a P4 switch. 
We illustrate the anomalies in the switch behavior due to missing checks in the publicly available P4 programs from P4 tutorial solutions~\cite{p4tut} and NetPaxos~\cite{netp} codebase.
 
%In this section we show a small example of some simple possible errors in a P4 program can have a critical effects even on the security of the system. Such a  problem may appear in syntactically correct, perfectly running code. If the P4 target device acts as a firewall, we can safely assume that it uses some kind of acl to filter traffic. As P4 programs execute actions on a packet based on a match-action tables. In Figure \ref{fig:missplacedacl} we can see a miss-placed application of the acl. In this case the acl will only apply to packets with valid IPv$4$ headers. This way IPv$6$ packets could be used to start an attack against the defended network.
%However, this is not the only problem regarding the code snippet in Figure \ref{fig:missplacedacl}. As "if" statements cannot be used in actions in P$4$, some additional considerations should take place on the mentioned figure. If an attacker intercepts and modifies an encrypted packet meant for the system in question, the checksum value most probably will be wrong. However, as the firewall do not check this value (there is no "if" statement regarding this particular field), the firewall will forward it and correct the checksum, legalizing the packet. This gives an opportunity to an attacker to insert malicious pieces of code or information, and get it to the system without any problems. 
%To the best of our knowledge, such scenarios are non-trivial to debug by any of the existing static analysis-based P4 program debugging approaches~\cite{stoenescu2018debugging,liu2018p4v,neves2018verification}.Scenarios like checksum-related bugs (see Example Scenario 1) are non-trivial to debug by any of the existing static analysis-based P4 program debugging approaches~\cite{stoenescu2018debugging,liu2018p4v,neves2018verification}. TTL-related bugs (see Example Scenario 2) can be, however, detected by~\cite{stoenescu2018debugging,neves2018verification}Such scenarios can be easily reproduced in the official P4 tutorial program~\cite{p4tut}, e.g., \texttt{basic.p4} and the NetPaxos P4 program~\cite{netp}, e.g., \texttt{acceptor.p4}.

Software bugs or errors can occur at any stage in the P4 processing pipeline: parser, ingress match-action, packet replication engine (\texttt{PRE}), egress match-action, deparser and buffer queuing engine ((\texttt{BQE}). Note all stages except the PRE and BQE, are P4 programmable while PRE and BQE remain as a vendor specific, fixed function component. Figure~\ref{fig:mot2} illustrates the target device-dependent (in green) and -independent (in yellow) blocks in the \new packet processing pipeline. Note that the target device-independent blocks are programmable.

There can be, however, bugs in the parser code, e.g., when not or incorrectly checking the header fields, such as IPv4 header length (\texttt{ihl}) or \texttt{TTL} field. 
%In case the programmer, e.g., forgets to verify TTL field is greater than 0, decrementing the TTL results in a TTL of 255. 
%The checksum validation block in ingress match-action also possesses weaknesses, possibly accepting packets with wrong checksums.
% In case the programmer, e.g., does not choose to parse IPv4 packets with options, the resulting checksum calculation will be wrong, leading to packet drop at other hops in the network. 
As an example, consider the scenario in Figure~\ref{fig:mot2} (yellow blocks) that illustrates part of the implementation of L3 (Layer-3) switch, provided in the P4 language tutorial solutions~\cite{p4tut}. Here, the parser accepts any kind of IPv4 packets and does not check if the IPv4 header contains IPv4 options or not, i.e., if IPv4 \texttt{ihl} field is not or is equal to 5. When updating the IPv4 \texttt{checksum} of the packets during egress processing, IPv4 options are not taken into account, hence for those IPv4 packets with options, the resulting \texttt{checksum} is wrong causing such packets to be \textit{incorrectly} forwarded instead of getting dropped. This leads to anomaly in the network behavior.
%Therefore, the next hop in the network expected to drop such packets does not drop them, leading to anomaly in the network behavior. 
Currently, the detection of such runtime bugs is non-trivial. We call such errors as \textit{target device-independent bugs}, as these only result from programming errors involving one of the P4 programmable stages. 

These are, however, not the only kind of bugs that can occur. The interaction of the P4 program with the \texttt{PRE} may result in an unintended behavior as well, which we call as \textit{target device-dependent bugs}. The \texttt{PRE} is responsible for carrying out several forwarding actions, such as \texttt{clone}, \texttt{multicast}, \texttt{resubmit} or \texttt{drop}. The programmer uses standard metadata to communicate the forwarding action to the \texttt{PRE}, which interprets it and executes the actions accordingly. It is, however, very common to have situations where conflicting forwarding actions are selected. %Consider a scenario where a P4 program implementing at least two tables, where one could be an IPv4 longest prefix match (\texttt{LPM}) table and a following table an access control list (\texttt{ACL}). If packets are matched by the \texttt{LPM} table and a clone decision is made, those packets later, get dropped by the \texttt{ACL} table. In such a case, the forwarding behavior depends on the implementation of the \texttt{PRE}, which is target device-dependent. The implementation of \texttt{PRE} of the simple switch target in the behavioral model (Bmv2) would drop the original packet, however, \textit{incorrectly} forward the cloned copy of the packet. Similar runtime bugs can be seen, if instead of \texttt{clone}, \texttt{multicast} or \texttt{resubmit} actions are chosen.
As an example, consider the scenario shown in Figure~\ref{fig:mot2} (green blocks). Here, we assume a P4 program implementing at least two match-action tables. Any table except the last one could be a longest prefix match (\texttt{LPM}) table, offering unicast, clone and drop actions. The last match-action table implements an access control list (\texttt{ACL}). So, the packets can either be dropped or forwarded according to the chosen actions by the previous tables. In this case, it is possible that conflicting forwarding decisions are made. Consider packets matched by the first table and a clone decision is made, are later dropped by the \texttt{ACL} table. In such a case, the forwarding behavior depends on the implementation of the \texttt{PRE}, which is target device-dependent. The implementation of \texttt{PRE} of the simple switch target in the behavioral model (Bmv2) is illustrated in Figure~\ref{fig:mot2}. It would drop the original packet, however, forward the cloned copy of the packet. Similar bugs can be seen, if instead of the clone action, the resubmit action is chosen (in blue). Similarly, another bug can be found when implementing multicast (in green). 
%Furthermore, if the programmer does not decide to choose a forwarding action at all, the value of the \texttt{egress\_spec} field is undefined as per $P4_{16}$ specification~\cite{p4-specs}. Therefore, the hardware implementing \texttt{PRE} is allowed to return an arbitrary value for the \texttt{egress\_spec}, thus defining an arbitrary output port for such packets. 

\ap{Check}Target device-independent or -dependent bugs are present in many real-world P4 applications. Currently, some of the aforementioned runtime bugs such as checksum-related bugs and platform-dependent bugs cannot be detected by the existing static analysis approaches~\cite{stoenescu2018debugging,liu2018p4v,neves2018verification,Neves:2018:VPP:3281411.3281421}.

\begin{figure*}[t]
\centering
\begin{subfigure}[l]{0.5\columnwidth}
\centering
\includegraphics[width=\columnwidth, height=4cm]{figures/p4_newest.pdf}
%\vspace{-.25em}
\subcaption{The patchable percentage of code increases for each P4 program from \old to \new. This plot is for bmv2 switch architecture~\cite{bmv2}, i.e., it does not include explicit ingress deparser and egress parser. \label{fig:apps}}
%\vspace{-.25em}
\end{subfigure}%
\hspace{0.01\textwidth}
\begin{subfigure}[c]{0.5\columnwidth}
\centering
\includegraphics[width=\columnwidth, height=4cm]{figures/p4_explicit_new.pdf}
%\vspace{-.25em}
\subcaption{The patchable percentage of code increases for each P4 program from \old to \new. This plot is for generic PSA switch architectures~\cite{psasec,psaing} like Tofino~\cite{tofino}, i.e., includes explicit ingress deparser and egress parser.\label{fig:apps1}}
%\vspace{-.25em}
\end{subfigure}%
\hspace{0.01\textwidth}
\begin{subfigure}[r]{0.5\columnwidth}
\centering
\includegraphics[width=\columnwidth, height=4cm]{figures/bargraph_newest.pdf}
%\vspace{-.25em}
\subcaption{The patchable percentage of code for bmv2 switch architecture~\cite{bmv2}, i.e., it does not include explicit ingress deparser and egress parser in all different \new programs from P4 tutorials~\cite{p4tut}, NetPaxos~\cite{netp}.\label{fig:per}}
%\vspace{-.25em}
\end{subfigure}
\hspace{0.01\textwidth}
\begin{subfigure}[r]{0.5\columnwidth}
\centering
\includegraphics[width=\columnwidth, height=4cm]{figures/bargraph_explicit_new.pdf}
%\vspace{-.25em}
\subcaption{The patchable percentage of code for generic PSA switch architectures~\cite{psasec,psaing} like Tofino~\cite{tofino}, i.e., includes explicit ingress deparser and egress parser in all different \new programs from P4 tutorials~\cite{p4tut}, NetPaxos~\cite{netp}. \label{fig:per1}}
%\vspace{-.25em}
\end{subfigure}
\caption{Evolution of the P4 program structure from \old to \new version. Note calculator (calc) application from~\cite{p4tut} is not included here as it not a networking application.}
\label{fig:struct}
\vspace{.5em}
\end{figure*}
\begin{comment}
\begin{figure}[t]
\centering
%\includegraphics[width=\linewidth]{figures/scenario_v5-crop.pdf}
\includegraphics[width=0.9\columnwidth]{figures/figure_clone_v8-crop.pdf}
\caption{Example of a target device-dependent bug.}
%\ap{Make queries in different colour}}
\label{fig:mot2}
\end{figure}
\end{comment}
\subsection{Opportunities: Structure of a P4 program}
P4~\cite{bosshart2014p4,p416specs} is a domain-specific language comprising of packet-processing abstractions, e.g., headers, parsers, tables, actions, and controls. A simple abstract forwarding model is followed with five distinct
phases while executing a P4 program: \texttt{parsing}, \texttt{ingress processing}, \texttt{replication} and \texttt{queuing},
\texttt{egress processing}, and \texttt{deparsing}~\cite{bosshart2013forwarding}. The behavior of each of these phases is defined through declarations in a P4 program. 

The parser transforms the packet from bits into headers according to a parser specification provided by the programmer. After parsing, an ingress control function decides how the packet will be processed. Then, the packed is queued for egress processing. Upon dequeuing, it is processed by an egress control function. The deparser specification dictates how packets are deparsed from separate headers into a bit representation on output, and finally, the packet leaves the switch. Note that both ingress and egress control functions direct the packet through any number of match-action tables. Figure~\ref{fig:mot2} illustrates these stages of the P4 packet processing pipeline.%The control functions conditionally steer the packet to various tables based on header values, metadata or table match outcomes. %; packet contents cannot be changed in the control function. %During execution, the state comprises the data extracted from packet headers, metadata supplied by the device (e.g., the ingress port that the packet arrived on) or computed by the program, as well as mutable state in counters and registers.

Currently, P4 offers 2 versions: \old~\cite{p414specs} and \new~\cite{p416specs}. \new allows programmers to use definitions of a target switch-specific architecture, PSA (Portable Switch Architecture)~\cite{psasec,psaing} which is a target architecture that describes common capabilities of network switch devices. \new is an upgraded version of \old. In particular, a large number of language features have been eliminated from \old and moved into libraries including counters, checksum units, meters, etc. in \new. \old allowed the programmer to explicitly program three blocks: ingress parser (including header definitions of accepted header layouts), ingress control and egress control functions. As illustrated in Figure~\ref{fig:mot2}, \new allows to explicitly program six blocks: ingress parser (including header definitions of accepted header layouts), ingress control, ingress deparser, egress parser, egress control functions, and egress deparser.

We realize that as more blocks of the P4 program get programmable, there is more onus on the programmer to write a program that behaves as expected when it gets compiled and is deployed on the P4 switch. However, missing checks or manual errors can cause havoc in the network. However, this is also a blessing in disguise as the more programmable the code is, the more patchable it gets. Thus, the manual errors can be fixed. Figure~\ref{fig:per},~\ref{fig:per1} illustrate that the patchable code percentage increases from \old to \new in all applications (excluding calculator) from P4 tutorial solutions~\cite{p4tut} and NetPaxos codebase~\cite{netp} in behavioral model (bmv2) switch architecture~\cite{bmv2} and other generic PSA switch architectures~\cite{psasec,psaing}, e.g., Tofino~\cite{tofino} respectively.\\ 
\emph{\textbf{Observation 1:} From} \old \emph{to} \new, P4 \emph{program gets more complex as there are twice as more programmable blocks.}

Figure~\ref{fig:apps},~\ref{fig:apps1} illustrate the patchable code percentage in the latest \new version. The patchable code percentage comes from the six programmable blocks in \new. Roughly, whatever is programmable, is patchable. In particular, around 40-45\% of a P4 program is patchable in \new programs for behavioral model (bmv2) switch architecture~\cite{bmv2} (Figure~\ref{fig:apps}). This increases to 50-55\% if the ingress deparser and egress parser is programmable for other target switch architectures, e.g., Tofino~\cite{tofino} (Figure~\ref{fig:apps1}). More importantly, the parser and header definitions account for 20-40\% of the total patchable code. Therefore, if there is no bug in the parser and header code, the runtime behavior of the switch running the compiled P4 program to the incoming packets should more or less behave as expected.\\ 
\emph{\textbf{Observation 2:} Parser code is patachable if localized; else the unexpected incoming traffic may get rejected anyway; otherwise the bug lies in the target-device dependent part or other parts of P4 code.} 

%see Figure~\ref{fig:per}\\
\begin{comment}
\begin{figure}[t]
\centering
%\includegraphics[width=\linewidth]{figures/apps.jpg}
\includegraphics[width=\columnwidth]{figures/p4_new.pdf}
\caption{The patchable percentage of code increases for each P4 program from \old to \new.}
%\ap{Make queries in different colour}}
\label{fig:apps}
\end{figure}
\begin{itemize}
    \item \new allows to explicitly program parser and deparser of the different stages (Ingress/ Egress) in the processing pipeline.
    \item Depending on the switch architecture the programmer needs to explicitly program both parser and deparser for each stage, ingress and egress.
    \item E.g. portable switch architecture (PSA) requires to explicitly program ingress parser, ingress deparser, egress parser and egress deparser~\cite{psaing,psasec}
    \item Bmv2 simple switch architecture is based on an architecture model that only requires the programmer to program ingress parser and egress deparser.
\end{itemize}
%see Figure~\ref{fig:apps}\\

%\emph{\textbf{Observation3:} other parts of code}

\begin{figure}[t]
\centering
%\includegraphics[width=\linewidth]{figures/Percent.jpg}
\includegraphics[width=\columnwidth]{figures/bargraph_new.pdf}
\caption{The patchable percentage of code in ten different \new programs from P4 tutorials~\cite{p4tut} and NetPaxos~\cite{netp} codebase.}
%\ap{Make queries in different colour}}
\label{fig:per}
\end{figure}
\end{comment}

